Structured and Decorated Cospans from the Viewpoint of Double Category Theory

Structured and decorated cospans are broadly applicable frameworks for building bicategories or double categories of open systems. We streamline and generalize these frameworks using central concepts of double category theory. We show that, under mild hypotheses, double categories of structured cospans are cocartesian (have finite double-categorical coproducts) and are equipments. The proofs are simple as they utilize appropriate double-categorical universal properties. Maps between double categories of structured cospans are studied from the same perspective. We then give a new construction of the double category of decorated cospans using the recently introduced double Grothendieck construction. Besides its conceptual value, this reconstruction leads to a natural generalization of decorated cospans, which we illustrate through an example motivated by statistical theories and other theories of processes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{210}
\providecommand{\publicationstatus}{S. Staton, C. Vasilakopoulou (Eds.):\\
Applied Category Theory 2023 (ACT2023)\\
EPTCS 397, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.397.13}{10.4204/EPTCS.397.13}}
\pdfoutput=1

